On Differentially Private Federated Linear Contextual Bandits

We consider cross-silo federated linear contextual bandit (LCB) problem under differential privacy, where multiple silos (agents) interact with the local users and communicate via a central server to realize collaboration while without sacrificing each user's privacy. We identify three issues in the state-of-the-art: (i) failure of claimed privacy protection and (ii) incorrect regret bound due to noise miscalculation and (iii) ungrounded communication cost. To resolve these issues, we take a two-step principled approach. First, we design an algorithmic framework consisting of a generic federated LCB algorithm and flexible privacy protocols. Then, leveraging the proposed framework, we study federated LCBs under two different privacy constraints. We first establish privacy and regret guarantees under silo-level local differential privacy, which fix the issues present in state-of-the-art algorithm. To further improve the regret performance, we next consider shuffle model of differential privacy, under which we show that our algorithm can achieve nearly ``optimal'' regret without a trusted server. We accomplish this via two different schemes -- one relies on a new result on privacy amplification via shuffling for DP mechanisms and another one leverages the integration of a shuffle protocol for vector sum into the tree-based mechanism, both of which might be of independent interest. Finally, we support our theoretical results with numerical evaluations over contextual bandit instances generated from both synthetic and real-life data.

==> vecsum.tex <==







% \begin{algorithm}
% \caption{${P}_{\text{vec}}$, a shuffle protocol for vector summation \cite{cheu2021shuffle}}
% \label{alg: Pvec}
% \begin{algorithmic}[1]
% \STATE {\bfseries Input:} database of $d$-dimensional vectors $\mathbf{X}= (\mathbf{x}_1, \cdots, \mathbf{x}_N$); privacy parameters $\epsilon, \delta$; $L$.
% %
% \STATE {\bfseries procedure:} Local Randomizer $\mathcal{R}_{\text{vec}}(\mathbf{x}_i)$
% \begin{ALC@g}
% \FOR{$j \in [d]$} 
% \STATE Shift component to enforce non-negativity: $\mathbf{w}_{i,j} \gets \mathbf{x}_{i,j} + L$
% \STATE $\mathbf{m}_j \gets \mathcal{R}_{1D}(\mathbf{w}_{i,j})$
% \ENDFOR
% \STATE Output labeled messages $\{(j, \mathbf{m}_j)\}_{j \in [d]}$
% \end{ALC@g}
% \STATE {\bfseries end procedure}
% \STATE {\bfseries procedure: Analyzer} $\mathcal{A}_{\text{vec}}(\mathbf{y})$ 
% \begin{ALC@g}
% \FOR{$j \in [d]$}
% \STATE Run analyzer on coordinate $j$'s messages $z_j \gets \mathcal{A}_{\text{1D}}(\mathbf{y}_j)$ 
% \STATE Re-center: $o_j \gets z_j - N \cdot L$
% \ENDFOR
% \STATE Output the vector of estimates $\mathbf{o} = (o_1, \cdots o_d)$
% \end{ALC@g}
% \STATE {\bfseries end procedure}
% \end{algorithmic}
% \end{algorithm}
